Ordinal Regression via Binary Preference vs Simple Regression: Statistical and Experimental Perspectives

Ordinal regression with anchored reference samples (ORARS) has been proposed for predicting the subjective Mean Opinion Score (MOS) of input stimuli automatically. The ORARS addresses the MOS prediction problem by pairing a test sample with each of the pre-scored anchored reference samples. A trained binary classifier is then used to predict which sample, test or anchor, is better statistically. Posteriors of the binary preference decision are then used to predict the MOS of the test sample. In this paper, rigorous framework, analysis, and experiments to demonstrate that ORARS are advantageous over simple regressions are presented. The contributions of this work are: 1) Show that traditional regression can be reformulated into multiple preference tests to yield a better performance, which is confirmed with simulations experimentally; 2) Generalize ORARS to other regression problems and verify its effectiveness; 3) Provide some prerequisite conditions which can insure proper application of ORARS.

==> secRelated.tex <==
\section{Related Work}
Subjective assessment is to assess the input stimuli based on an ordinal scale, like \{bad, poor, average, good, excellent\}. It is a typical "assessing ordered categorical variables" task. As \cite{gutierrez2015ordinal} suggested, ordinal regression could be used to solve this problem. 

Speech fluency assessment is a specific subjective assessment task which assess how fluent of a given speech is. \cite{mao2019nn} proposed Ordinal Regression with Anchored Reference Samples (ORARS) to solve it. 

The main idea is comparing the test samples with pre-scored anchored reference samples, then scoring the test sample according to the comparsion result. The framework is shown as Fig.\ref{fig:framework}. The framework contains two components, i.e, a binary classifier $g$ to predict statistically which sample, test or anchor,is better and a scoring module $h$ to predict the final score.

In detail, the training set $\mathbf{D}$ is separated into two disjoint subsets, i.e, anchor set $\mathbf{D_A}$ and training set $\mathbf{D_T}$ where anchor set contains $N_A$ samples in each rank. The binary classifier is trained on the cartesian product of $\mathbf{D_A}$ and $\mathbf{D_T}$.  Let $x_t$ and $x_a$ be the two samples' features from $\mathbf{D_T}$ and $\mathbf{D_A}$, and croresponding labels are $y_t$ and $y_a$, respectively. The binary classifier is training with the concatenation of $x_t$ and $x_a$ as input feature, and croresponding label is calcuated as Eq.\ref{eq:get_label}
\begin{equation}
    label=\left\{
    \begin{aligned}
    1\quad& y_t>y_a \\
    0\quad& y_t\le y_a 
    \end{aligned}
    \right.
    \label{eq:get_label}
\end{equation}

When the binary classifier is trained, the score of test sample whose feature is denoted as $x$ is determined by Eq.\ref{eq:mao_score}
\begin{equation}
    s=\frac{\sum_{k=1}^K\sum_{a=1}^{N_A}g(x,x_a^k)}{N_A}
    \label{eq:mao_score}
\end{equation}
where $k$ deonte the rank where the anchor sample from and $x_a^k$ is the anchor feature from $k$-th rank. The output of binary classifier is regarded as confidence of $y_t>y_a$. Since the decision of $g$ is soft, the model can predict a continus target value. 

The limition of \cite{mao2019nn} proposed model is that require each rank contain $N_A$ samples at least which may can not be satisfied in real dataset. \cite{su2020improving} improves the ORARS by modifing the scoring method. To train ORARS on dataset with any label distribution, there's no specific anchor set. The binary classifier is trained on the self-cartesian product of $\mathbf{D}$, all training set is used as anchor set when inference stage. The new ORARS score given test sample as $r$-th largest score in training set. Although the scoring method proposed by \cite{su2020improving} was applied on a discrete target value, it is easy to apply it on a continuous target value.

In addition, \cite{su2020improving} the binary classifier is trained with a weight function which is shown as Eq.\ref{eq:su_weight}
\begin{equation}
    w=min(|y_1-y_1|,1)
    \label{eq:su_weight}
\end{equation}

The new ORARS shows its ability on speech pronunciation assessment. 

This article is interested in using ORARS to solve general regression problems, if it is possible, the reason is worth thinking about.


